Hybrid Automated Program Repair by Combining Large Language Models and Program Analysis

Automated Program Repair (APR) has garnered significant attention due to its potential to streamline the bug repair process for human developers. Recently, LLM-based APR methods have shown promise in repairing real-world bugs. However, existing APR methods often utilize patches generated by LLMs without further optimization, resulting in reduced effectiveness due to the lack of program-specific knowledge. Furthermore, the evaluations of these APR methods have typically been conducted under the assumption of perfect fault localization, which may not accurately reflect their real-world effectiveness. To address these limitations, this paper introduces an innovative APR approach called GIANTREPAIR. Our approach leverages the insight that LLM-generated patches, although not necessarily correct, offer valuable guidance for the patch generation process. Based on this insight, GIANTREPAIR first constructs patch skeletons from LLM-generated patches to confine the patch space, and then generates high-quality patches tailored to specific programs through context-aware patch generation by instantiating the skeletons. To evaluate the performance of our approach, we conduct two large-scale experiments. The results demonstrate that GIANTREPAIR not only effectively repairs more bugs (an average of 27.78% on Defects4J v1.2 and 23.40% on Defects4J v2.0) than using LLM-generated patches directly, but also outperforms state-of-the-art APR methods by repairing at least 42 and 7 more bugs under perfect and automated fault localization scenarios, respectively.

==> alg/filling.tex <==
\begin{algorithm}
\caption{Filling Skeleton}
\label{algo:mutation}
\SetAlgoLined
\SetKwProg{Fn}{Func}{:}{}
\SetKwFunction{FFillSkeleton}{FillSkeleton}
\Fn{\FFillSkeleton{sk: Skeleton}}{
$candidates \leftarrow Fill(sk, null)$\\
$patches \leftarrow$  apply candidates to buggy code\\
\KwRet{patches}
}

\SetKwFunction{FFill}{Fill}
\Fn{\FFill{$n: ASTNode, type:String$}}{
$result \leftarrow \varnothing$\\
\If{$n.children == null$}{
$result \leftarrow $ get accessible candidate from scopes\\
\KwRet{$result$}
}
\For{$child$ in $n.children$}{
$candidates \leftarrow Fill(child, requiredType)$\\
$newNodes \leftarrow $ apply all candidates on $n$\\
$result \leftarrow result \cup newNodes$
}
\KwRet{$result$}
}
\end{algorithm}

==> alg/static_analysis.tex <==
\begin{algorithm}
\caption{Static Analysis}
\label{algo:static_analysis}
\SetAlgoLined
\SetKwProg{Fn}{Func}{:}{}
\SetKwFunction{FStatic}{staticAnalysis}
\SetKwFunction{FAnalyze}{analyze}
\Fn{\FStatic{f: Buggy file}}{
$files = ExtractRelated(f)$ \\
$scopes \leftarrow \varnothing$\\
\For{$file$ in $files$}{
$scope \leftarrow new$ $Scope(file.className)$\\
$analyze(file.root, scope)$\\
$scopes.add(scope)$
}
\KwRet{$scopes$}
}

\Fn{\FAnalyze{node: ASTNode, scope: Scope}}{
$newScope \leftarrow \varnothing$\\
\If{$node.type == Block$}{
$newScope \leftarrow new $ $Scope()$\\
$scope.addChild(newScope)$\\
$scope = newScope$\\
}
\If{$node.type == MethodDeclaration$}{
$scope.addMethod(method.signature)$\\
}
\If{$node.type == varDeclaration$}{
$scope.addVar(<type, isStatic, name>)$
}
\For{$child in node.children$}{
$analyze(child, scope)$\\
}
\KwRet{$scope$}
}
\end{algorithm}

==> tables/Table_4_Contribution.tex <==
% \begin{table}[htbp]
%     \caption{Component contribution of \TOOL{}\jiajun{May use histogram.} \jiajun{Based on this table, the abstraction process is related to these node types? If yes, can we summarize a table to show the abstraction strategy for each of them? such as the table title is ``Node Type, example, Skeleton'' and an example is ``MethodInovation, a.function(b), \_var[T1].\_func(\_var[T2])'', where ``\_var'' denotes variable placeholder, ``\_func'' denotes method name placeholder, while ``T1'' and ``T2'' are the type constraints for corresponding ``\_var''. Then, we can instantiate the patches based on these constraints.}}
%     \label{tab:table_4_contribution}
%     \centering
%     \begin{tabular}{ccc}
%         \hline
%         % \multirow{2}{}{}
%         \makecell{Filling Strategy} & \makecell{\#Relevant\\Correct Fixes} & \%Percentage\\
%         \hline
%         MethodInvocation&27&64.29\\
%         IfStatement&22&52.38\\
%         ReturnStatement&11&26.19\\
%         InfixExpression&11&26.19\\
%         ExpressionStatement&7&16.67\\
%         PrefixExpression&5&11.9\\
%         Block&5&11.9\\
%         ConstructorInvocation&4&9.52\\
%         ClassInstanceCreation&3&7.14\\
%         ThrowStatement&2&4.76\\
%         Assignment&2&4.76\\
%         ForStatement&1&2.38\\
%         BooleanLiteral&1&2.38\\
%         SimpleName&1&2.38\\
%         \hline
%         % \textbf{Total} & \multicolumn{2}{c}{103}\\
%         % \hline
%     \end{tabular}
% \end{table}

% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%     \begin{axis}[
%         ybar,
%         enlargelimits=0.08,
%         legend style={at={(0.5,-0.15)},
%           anchor=north,legend columns=-1},
%         ylabel={times},
%         symbolic x coords={MethodInvocation, IfStatement, ReturnStatement, InfixExpression, ExpressionStatement, PrefixExpression, ConstructorInvocation, ClassInstanceCreation, ThrowStatement, Assignment, ForStatement, BooleanLiteral, SimpleName},
%         xtick=data,
%         nodes near coords,
%         nodes near coords align={vertical},
%         enlarge y limits={upper,value=0.2}, % 谉整Y轴的上边界
%         x tick label style={rotate=45, anchor=east}, % 倾斜X轴标签
%     ]
% \addplot[fill={rgb:red,1;green,2;blue,3}] coordinates {(MethodInvocation,27) (IfStatement,22) (ReturnStatement,11) (InfixExpression,11) (ExpressionStatement,7) (PrefixExpression, 5) (ConstructorInvocation, 4) (ClassInstanceCreation, 3) (ThrowStatement, 2) (Assignment, 2) (ForStatement, 1) (BooleanLiteral, 1) (SimpleName, 1) };
% % \legend{show1}
% \end{axis}
% \end{tikzpicture}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

==> tables/Table_5_SBFL.tex <==
\begin{table}[htbp]
    \label{tab:table_4_contribution}
    \caption{n \TOOL{}'s correct fixes without Perfect Fault Localization}
    \centering
    \begin{tabular}{cccccc}
        \hline
        % \multirow{2}{}{}
         \TOOL{} & Tare& Recoder & DLFix & TBar & SimFix\\
        \hline 
        69 & 57 & 49 & 30 & 42 & 34\\
        \hline
        % \textbf{Total} & \multicolumn{2}{c}{103}\\
        % \hline
    \end{tabular}
\end{table}

==> tables/Table_6_gpt4.tex <==
\begin{table*}[htbp]
    \caption{Comparsion with GPT-4-1106-preview}
    \label{tab:table_6_gpt4}
    \centering
    \footnotesize
    \begin{tabular}{c|cccccccccc}
    \toprule
    \textbf{Bug ids} & \textbf{Closure-19} & \textbf{Closure-36} & \textbf{Closure-113} & \textbf{Lang-57} & \textbf{Math-27} & \textbf{Math-85} & \textbf{Cli-32} & \textbf{Codec-4} & \textbf{Compress-1} & \textbf{Jsoup-33} \\
    \midrule
    GPT-4-1106-preview & \checkmark & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
    \hline
    \TOOL{} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/Table_7_growing.tex <==
\begin{table}[htbp]
    \caption{Correct Fixes on GrowingBugs}
    \label{tab:table_7_growing}
    \centering
    \small
    \begin{tabular}{ccc}
    \toprule
    Project & Bugs\#SF & \TOOL{} \\
    \midrule
    Canvas\_api & 2 & 1 \\
    Dosgi\_common & 1 & 1 \\
    Hono\_client & 2 & 0 \\
    Tika\_app & 1 & 1 \\
    HttpClient5 & 2 & 0 \\
    JacksonDatatypeJsr310 & 1 & 0 \\
    JacksonModuleAfterburner & 1 & 1 \\
    Switchyard\_admin & 1 & 1\\
    Qpidjms\_client & 1 & 0 \\
    Tiles\_api & 1 & 0\\
    Tiles\_core & 2 & 0\\
    Wicket\_request & 5 & 0 \\
    Wicket\_util & 4 & 1 \\
    Wicket\_spring & 1 & 0\\
    Struts1\_core & 2 & 0 \\
    Wicket\_core & 10 & 2 \\
    Cargo\_container & 3 & 0 \\
    Jcodemodel & 1 & 1\\
    Vectorz & 2 & 0 \\
    Restfixture & 2 & 0\\
    Xades4j & 1 & 0 \\
    Render\_app & 1 & 0 \\ 
    Leshan\_core & 4 & 1\\
    \midrule
    Total & 51 & 10\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/Table_8_toolList.tex <==
\begin{table}[htb]
    \centering
    \caption{Overview of compared baselines}
    \label{tab:my_label}
    \begin{tabular}{c|c|c||c|c|c}
    \toprule
        \textbf{Tool} & \textbf{Year} & \textbf{Venue} & \textbf{TOOl} & \textbf{Year} & \textbf{Venue} \\
    \hline
         Tare& 2023 & ICSE & TBar& 2019 & ISSTA \\
         Knod& 2023 & ICSE & Prapr& 2019 & ASE \\
         FitRepair& 2023 & ASE & Avatar & 2019 & SANER \\
         Repilot& 2023 & FSE & SimFix& 2018 & ISSTA \\
         GAMMA& 2023 & ASE & CapGen& 2018 & ICSE \\
         AlphaRepair& 2022 & FSE & SketchFix & 2018 & ICSE\\
         Hanabi& 2022 & TOSEM & JAID & 2017 & ASE \\
         SelfAPR& 2022 & ASE & jGenProg & 2017 & ESE\\
         Recoder& 2021 & FSE & jKali & 2016 & ISSTA \\
         CURE& 2021 & ICSE & jMutRepair& 2016 & ISSTA\\
         FixMiner& 2020 & ESE & NOPOL & 2014 & -\\
    \end{tabular}
\end{table}
